The trigger slow control system of the Belle II experiment

The Belle II experiment at the SuperKEKB $e^{+}e^{-}$ collider in KEK, Japan, started physics data-taking with a complete detector from early 2019 with the primary physics goal of probing new physics in heavy quark and lepton decays. An online trigger system is indispensable for the Belle II experiment to reduce the beam background events associated with high electron and positron beam currents without sacrificing the target physics-oriented events. During the Belle II operation upon beam collision, the trigger system must be consistently controlled and its status must be carefully monitored in the process of data acquisition against unexpected situations. For this purpose, we have developed a slow control system for the Belle II trigger system. Around seventy thousand configuration parameters are saved in the Belle II central database server for every run when a run starts and stops. These parameters play an essential role in offline validation of the quality of runs. Around three thousand real-time variables are stored in the Belle II main archiving server, and the trend of some of these variables are regularly used for online and offline monitoring purposes. Various operator interface tools have been prepared and used. When the configuration parameters are not correctly applied, or some of the processes are unexpectedly terminated, the slow control system detects it, stops the data-taking process, and generates an alarm. In this article, we report how we constructed the Belle II trigger slow control system, and how we successfully managed to operate during its initial stage.

==> log.tex <==
%% 
%% Copyright 2007-2019 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% ---------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%% 
%% given in the file `manifest.txt'.
%% 
%% Template article for Elsevier's document class `elsarticle'
%% with harvard style bibliographic references



%%%%% Cheolhun Kim

%%%%% 2021.01.13(THR) ver8.00: arXiv and NIMA submit version.


%%%%% 2021.01.20(WED) unnecessary figures are removed. 
%%%%% 2021.01.13(THR) ver7.02: final version (before submission) started.


%%%%% 2021.01.12(WED) minor mistakes are edited. Fig. 3 updated.
%%%%% 2021.01.12(WED) ver7.00 started.


%%%%% 2021.01.12(WED) Fig 6. updated: cosmic runs => cosmic-ray runs
%%%%% 2021.01.11(MON) ver7.00 started. Nakao-san's final comments.


%%%%% 2020.12.14(MON) ver6.01 started. minor modifications.
%%%%% 2020.12.11(FRI) ver6.00 started. Nakao-san's comments.


%%%%% 2020.11.16(MON) Final! E-mail gogo to Nakao-san.
%%%%% 2020.11.16(MON) Final edition before sending an e-mail to Nakao-san.
%%%%% 2020.11.16(MON) Some plots are moved to another place (ver2). Nakao-san's comments.
%%%%% 2020.11.16(MON) All sections are reviewed. Nakao-san's comments.
%%%%% 2020.11.15(SUN) Section 3: Adding contents. Look through paper and edit. Nakao-san's comments.
%%%%% 2020.11.13(FRI) Add passion(?) continued, Look through paper and edit. Sectopm structure changed (latex only), Nakao-san's comments.
%%%%% 2020.11.11(WED) Add passion(?), Look through paper and edit. Nakao-san's comments.
%%%%% 2020.11.04(WED) ver5.01 started. Following rather complex comments (4). Nakao-san's comments.
%%%%% 2020.11.04(WED) ver5.01 started. Nakao-san's comments.


%%%%% 2020.10.16(FRI) ver5.00 started. Nakao-san's comments.
%%%%% 2020.10.30(FRI) Nakao-san's comments complete 18/24 (no nuisance)
%%%%% 2020.11.04(WED) Nakao-san's comments complete 24/24 (no nuisance)


%%%%% 2020.03.23(THU) ver3.02 started. Nakazawa-san's comments.

%%%%% 2020.03.12(THU) whole abstract, intro, summary, ref, Nakao-san's comments 24/25
%%%%% 2020.03.12(THU) ver3.01 started. Nakao-san's major comments.

%%%%% 2020.03.06(FRI) Oskar's comment: 40/41 => RC state/request table
%%%%% 2020.03.03(TUE) Oskar's comment 34/41 => Edit easy thing, first.
%%%%% 2020.03.03(TUE) Oskar's comment: abstract, intro - start, detector, TRG
%%%%% 2020.02.20(MON) ver3.00 started. Oskar's major comments.


%%%%% 2020.02.20(THU) Edit with Spruck's comments (Started, Completed.)
%%%%% 2020.02.20(THU) Edit by all Koga-san's comment: plot changed (Koga-san's BPAC slide plot)
%%%%% 2020.02.17(MON) ver2.02 started.


%%%%% 2020.02.17(MON) Edit by all Koga-san's comments (complete)
%%%%% 2020.02.17(MON) Edit based on Koga-san's comments
%%%%% 2020.02.17(MON) [Intro] In this paper, describe show => describe
%%%%% 2020.02.17(MON) ver2.01 started. 


%%%%% 2020.02.13(THU) Edit based on Nakao-san's minor comments. Major comments are edited later.
%%%%% 2020.02.13(THU) ver2.00 started.


%%%%% 2020.02.12(WED) updated // Edit abstract
%%%%% 2020.02.11(TUE) updated // Edit based on Insoo's comments, almost all, CH18 reference edit
%%%%% 2020.02.04(TUE) updated // Edit based on Insoo's comments, formula font
%%%%% 2020.01.30(THU) updated // Edit panels (ECLTRG part), user module => operator interface, acronyms, abstract(slightly edited)
%%%%% 2020.01.29(WED) updated // Edit panels (except ECLTRG)
%%%%% 2020.01.17(FRI) updated // Edit overview
%%%%% 2020.01.16(THU) updated // Edit Abstract, Introduction, Operation, Summary.
%%%%% 2020.01.15(WED) updated // GDL bits, Abstract, fig/table position.
%%%%% 2020.01.10(FRI) updated // Acknowlegement
%%%%% 2020.01.09(THU) updated // Author list. Reference numbering.
%%%%% 2019.12.12(THU) updated // Second full revision by myself, the L1 TRG rate and the ECL TRG luminosity / count are changed.
%%%%% 2019.12.10(TUE) updated // First full revision by myself.
%%%%% 2019.12.04(TUE) updated // First version is completed.
%%%%% ver1.00 started.


%%%%% 2019.11.22(FRI) updated // Overview, database explanation
%%%%% 2019.11.21(THU) updated // Overview, database list
%%%%% 2019.11.20(WED) updated // Overview, TRG SLC processes plot: explanation
%%%%% 2019.11.19(TUE) updated // Overview, TRG SLC processes plot.
%%%%% 2019.11.18(MON) updated // Overview, TRG SLC server structure plot.
%%%%% 2019.11.08(FRI) updated // Intro is edited. 
%%%%% 2019.11.01(FRI) updated // ver003 started. File separation.
%%%%% 2019.07.23(TUE) updated // Figure/table captions, on-going.
%%%%% 2019.07.22(MON) updated // Some figures are added.
%%%%% 2019.07.15(MON) updated // Archiver Table is added.
%%%%% 2019.07.03(TUE) updated
%%%%% 2019.07.02(TUE) created
%%%%% ver0.00 started.
